Unsupervised Traffic Scene Generation with Synthetic 3D Scene Graphs

Image synthesis driven by computer graphics achieved recently a remarkable realism, yet synthetic image data generated this way reveals a significant domain gap with respect to real-world data. This is especially true in autonomous driving scenarios, which represent a critical aspect for overcoming utilizing synthetic data for training neural networks. We propose a method based on domain-invariant scene representation to directly synthesize traffic scene imagery without rendering. Specifically, we rely on synthetic scene graphs as our internal representation and introduce an unsupervised neural network architecture for realistic traffic scene synthesis. We enhance synthetic scene graphs with spatial information about the scene and demonstrate the effectiveness of our approach through scene manipulation.

==> figure_cs_bdd_h.tex <==
\begin{figure*}[t!]
\begin{minipage}{0.325\textwidth}
\centering
\includegraphics[height=0.5\textwidth]{images/pfd2bdd/graphs/67.png}
\includegraphics[height=0.5\textwidth]{images/pfd2bdd/graphs/88.png}
\includegraphics[height=0.5\textwidth]{images/pfd2bdd/graphs/127.png}
\includegraphics[height=0.5\textwidth]{images/pfd2bdd/graphs/138.png}
\includegraphics[height=0.5\textwidth]{images/pfd2bdd/graphs/156.png}
\includegraphics[height=0.5\textwidth]{images/pfd2bdd/graphs/158.png}
% \includegraphics[height=0.5\textwidth]{images/pfd2bdd/graphs/171.png}
\includegraphics[height=0.5\textwidth]{images/pfd2bdd/graphs/217.png}
\caption*{SG}
\end{minipage}
\begin{minipage}{0.325\textwidth}
\includegraphics[width=1\textwidth]{images/pfd2bdd/images/67.png}
\includegraphics[width=1\textwidth]{images/pfd2bdd/images/88.png}
\includegraphics[width=1\textwidth]{images/pfd2bdd/images/127.png}
\includegraphics[width=1\textwidth]{images/pfd2bdd/images/138.png}
\includegraphics[width=1\textwidth]{images/pfd2bdd/images/156.png}
\includegraphics[width=1\textwidth]{images/pfd2bdd/images/158.png}
% \includegraphics[width=1\textwidth]{images/pfd2bdd/images/171.png}
\includegraphics[width=1\textwidth]{images/pfd2bdd/images/217.png}
\caption*{\textit{BDD}}
\end{minipage}
\begin{minipage}{0.325\textwidth}
\includegraphics[width=1\textwidth]{images/pfd2cs/images/67.png}
\includegraphics[width=1\textwidth]{images/pfd2cs/images/88.png}
\includegraphics[width=1\textwidth]{images/pfd2cs/images/127.png}
\includegraphics[width=1\textwidth]{images/pfd2cs/images/138.png}
\includegraphics[width=1\textwidth]{images/pfd2cs/images/156.png}
\includegraphics[width=1\textwidth]{images/pfd2cs/images/158.png}
% \includegraphics[width=1\textwidth]{images/pfd2cs/images/171.png}
\includegraphics[width=1\textwidth]{images/pfd2cs/images/217.png}
\caption*{\textit{CS}}
\end{minipage}
\caption{An example of traffic scene manipulation by changing spatial relation of 2 car }
\label{fig:joint_horizontal}
\end{figure*}

\begin{figure*}[t!]
\begin{minipage}{0.325\textwidth}
\centering
% \includegraphics[height=0.5\textwidth]{images/pfd2bdd/graphs/265.png}
% \includegraphics[height=0.5\textwidth]{images/pfd2bdd/graphs/276.png}
% \includegraphics[height=0.5\textwidth]{images/pfd2bdd/graphs/74.png} too wide
% \includegraphics[height=0.5\textwidth]{images/pfd2bdd/graphs/421.png}
% \includegraphics[height=0.5\textwidth]{images/pfd2bdd/graphs/422.png}
\includegraphics[height=0.5\textwidth]{images/pfd2bdd/graphs/444.png}
\includegraphics[height=0.5\textwidth]{images/pfd2bdd/graphs/465.png}
% \includegraphics[height=0.5\textwidth]{images/pfd2bdd/graphs/522.png}
% \includegraphics[height=0.5\textwidth]{images/pfd2bdd/graphs/562.png}
\includegraphics[height=0.5\textwidth]{images/pfd2bdd/graphs/574.png}
\includegraphics[height=0.5\textwidth]{images/pfd2bdd/graphs/623.png}
% \includegraphics[height=0.5\textwidth]{images/pfd2bdd/graphs/1660.png}
\includegraphics[height=0.5\textwidth]{images/pfd2bdd/graphs/1716.png}

\caption*{SG}
\end{minipage}
\begin{minipage}{0.325\textwidth}
% \includegraphics[width=1\textwidth]{images/pfd2bdd/images/265.png}
% \includegraphics[width=1\textwidth]{images/pfd2bdd/images/276.png}
% \includegraphics[width=1\textwidth]{images/pfd2bdd/images/74.png}
% \includegraphics[width=1\textwidth]{images/pfd2bdd/images/421.png}
% \includegraphics[width=1\textwidth]{images/pfd2bdd/images/422.png}
\includegraphics[width=1\textwidth]{images/pfd2bdd/images/444.png}
\includegraphics[width=1\textwidth]{images/pfd2bdd/images/465.png}
% \includegraphics[width=1\textwidth]{images/pfd2bdd/images/522.png}
% \includegraphics[width=1\textwidth]{images/pfd2bdd/images/562.png}
\includegraphics[width=1\textwidth]{images/pfd2bdd/images/574.png}
\includegraphics[width=1\textwidth]{images/pfd2bdd/images/623.png}
% \includegraphics[width=1\textwidth]{images/pfd2bdd/images/1660.png}
\includegraphics[width=1\textwidth]{images/pfd2bdd/images/1716.png}
\caption*{\textit{BDD}}
\end{minipage}
\begin{minipage}{0.325\textwidth}
% \includegraphics[width=1\textwidth]{images/pfd2cs/images/265.png}
% \includegraphics[width=1\textwidth]{images/pfd2cs/images/276.png}
% \includegraphics[width=1\textwidth]{images/pfd2cs/images/74.png}
% \includegraphics[width=1\textwidth]{images/pfd2cs/images/421.png}
% \includegraphics[width=1\textwidth]{images/pfd2cs/images/422.png}
\includegraphics[width=1\textwidth]{images/pfd2cs/images/444.png}
\includegraphics[width=1\textwidth]{images/pfd2cs/images/465.png}
% \includegraphics[width=1\textwidth]{images/pfd2cs/images/522.png}
% \includegraphics[width=1\textwidth]{images/pfd2cs/images/562.png}
\includegraphics[width=1\textwidth]{images/pfd2cs/images/574.png}
\includegraphics[width=1\textwidth]{images/pfd2cs/images/623.png}
% \includegraphics[width=1\textwidth]{images/pfd2cs/images/1660.png}
\includegraphics[width=1\textwidth]{images/pfd2cs/images/1716.png}
\caption*{\textit{CS}}
\end{minipage}
\caption{An example of traffic scene manipulation by changing spatial relation of 2 car }
\label{fig:joint_horizontal}
\end{figure*}

\begin{figure*}[t!]
\begin{minipage}{0.325\textwidth}
\centering
\includegraphics[height=0.5\textwidth]{images/pfd2bdd/graphs/726.png}
% \includegraphics[height=0.5\textwidth]{images/pfd2bdd/graphs/764.png}
\includegraphics[height=0.5\textwidth]{images/pfd2bdd/graphs/772.png}
\includegraphics[height=0.5\textwidth]{images/pfd2bdd/graphs/928.png}
\includegraphics[height=0.5\textwidth]{images/pfd2bdd/graphs/980.png}
\includegraphics[height=0.5\textwidth]{images/pfd2bdd/graphs/1001.png}
% \includegraphics[height=0.5\textwidth]{images/pfd2bdd/graphs/1074.png} too wide
% \includegraphics[height=0.5\textwidth]{images/pfd2bdd/graphs/1078.png} too wide
\includegraphics[height=0.5\textwidth]{images/pfd2bdd/graphs/1549.png}
\includegraphics[height=0.5\textwidth]{images/pfd2bdd/graphs/1566.png}
\includegraphics[height=0.5\textwidth]{images/pfd2bdd/graphs/1922.png}
\caption*{SG}
\end{minipage}
\begin{minipage}{0.325\textwidth}
\includegraphics[width=1\textwidth]{images/pfd2bdd/images/726.png}
% \includegraphics[width=1\textwidth]{images/pfd2bdd/images/764.png}
\includegraphics[width=1\textwidth]{images/pfd2bdd/images/772.png}
\includegraphics[width=1\textwidth]{images/pfd2bdd/images/928.png}
\includegraphics[width=1\textwidth]{images/pfd2bdd/images/980.png}
\includegraphics[width=1\textwidth]{images/pfd2bdd/images/1001.png}
% \includegraphics[width=1\textwidth]{images/pfd2bdd/images/1074.png}
% \includegraphics[width=1\textwidth]{images/pfd2bdd/images/1078.png}
\includegraphics[width=1\textwidth]{images/pfd2bdd/images/1549.png}
\includegraphics[width=1\textwidth]{images/pfd2bdd/images/1566.png}
\includegraphics[width=1\textwidth]{images/pfd2bdd/images/1922.png}
\caption*{\textit{BDD}}
\end{minipage}
\begin{minipage}{0.325\textwidth}
\includegraphics[width=1\textwidth]{images/pfd2cs/images/726.png}
% \includegraphics[width=1\textwidth]{images/pfd2cs/images/764.png}
\includegraphics[width=1\textwidth]{images/pfd2cs/images/772.png}
\includegraphics[width=1\textwidth]{images/pfd2cs/images/928.png}
\includegraphics[width=1\textwidth]{images/pfd2cs/images/980.png}
\includegraphics[width=1\textwidth]{images/pfd2cs/images/1001.png}
% \includegraphics[width=1\textwidth]{images/pfd2cs/images/1074.png}
% \includegraphics[width=1\textwidth]{images/pfd2cs/images/1078.png}
\includegraphics[width=1\textwidth]{images/pfd2cs/images/1549.png}
\includegraphics[width=1\textwidth]{images/pfd2cs/images/1566.png}
\includegraphics[width=1\textwidth]{images/pfd2cs/images/1922.png}
\caption*{\textit{CS}}
\end{minipage}
\caption{An example of traffic scene manipulation by changing spatial relation of 2 car }
\label{fig:joint_horizontal}
\end{figure*}

% \begin{figure*}[t!]
% \begin{minipage}{0.325\textwidth}
% \centering
% % \includegraphics[height=0.5\textwidth]{images/pfd2bdd/graphs/1414.png} too wide
% % \includegraphics[height=0.5\textwidth]{images/pfd2bdd/graphs/1592.png}
% % \includegraphics[height=0.5\textwidth]{images/pfd2bdd/graphs/1792.png} too wide
% \caption*{SG}
% \end{minipage}
% \begin{minipage}{0.325\textwidth}
% % \includegraphics[width=1\textwidth]{images/pfd2bdd/images/1414.png}
% % \includegraphics[width=1\textwidth]{images/pfd2bdd/images/1592.png}
% % \includegraphics[width=1\textwidth]{images/pfd2bdd/images/1792.png}
% \caption*{\textit{BDD}}
% \end{minipage}
% \begin{minipage}{0.325\textwidth}
% % \includegraphics[width=1\textwidth]{images/pfd2cs/images/1414.png}
% % \includegraphics[width=1\textwidth]{images/pfd2cs/images/1592.png}
% % \includegraphics[width=1\textwidth]{images/pfd2cs/images/1792.png} 
% \caption*{\textit{CS}}
% \end{minipage}
% \caption{An example of traffic scene manipulation by changing spatial relation of 2 car }
% \label{fig:joint_horizontal}
% \end{figure*}

==> figure_sg_layout_sm_pfd_cs.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.95\textwidth]{images_tmp/graph_with_background.png}
    \includegraphics[width=0.95\textwidth]{images_tmp/graph_proc_setup_2.png}
    \caption{Layouts (bottom) produced from the corresponding synthetic scene graphs (top) along with ground-truth layouts(middle). Colors follow Cityscapes protocol.}
    \label{fig:layouts1}
\end{figure*}

==> figure_teaser.tex <==
\begin{figure*}[t]
\begin{minipage}{1\columnwidth}
\includegraphics[width=0.75\textwidth]{images/scene_graph.png}
% \caption*{Original}
\end{minipage}
\begin{minipage}{1\columnwidth}
\includegraphics[width=1\textwidth]{images/sg_image_far.png}
\includegraphics[width=1\textwidth]{images/sg_image_close.png}
% \caption*{Original}
\end{minipage}
% \caption{\textbf{Caption}}\label{fig:teaser}
\end{figure*}

\begin{center}

\centering
% \includegraphics[width=0.325\textwidth]{images/pfd2bdd/graphs/74.png}
% \includegraphics[width=0.325\textwidth]{images/pfd2bdd/images/74.png}
% \includegraphics[width=0.325\textwidth]{images/pfd2cs/images/74.png}
% \captionof{figure}{Synthetic scene graph and generated traffic scenes from BDD (left) \cite{Yu2018} and Cityscapes (right) \cite{Cordts2016} datasets.}

\begin{minipage}{0.325\textwidth}
\centering
\includegraphics[width=1.1\textwidth]{images/pfd2bdd/graphs/74.png}
\includegraphics[width=1\textwidth]{images/pfd2bdd/images/74.png}
\includegraphics[width=1\textwidth]{images/pfd2cs/images/74.png}
% \caption*{Original}
\end{minipage}
\begin{minipage}{0.325\textwidth}
\centering
\includegraphics[height=0.5\textwidth]{images/pfd2bdd/graphs/562.png}
\includegraphics[width=1\textwidth]{images/pfd2bdd/images/562.png}
\includegraphics[width=1\textwidth]{images/pfd2cs/images/562.png}
% \caption*{Original}
\end{minipage}
\begin{minipage}{0.325\textwidth}
\centering
\includegraphics[height=0.5\textwidth]{images/pfd2bdd/graphs/88.png}
\includegraphics[height=0.5\textwidth]{images/pfd2bdd/images/88.png}
\includegraphics[height=0.5\textwidth]{images/pfd2cs/images/88.png}
% \caption*{Original}
\end{minipage}
\captionof{figure}{BDD and Cityscapes traffic scenes generated from synthetic scene graph.}\label{fig:teaser}
\end{center}

==> plot_neural_net/_net <==
\usetikzlibrary{positioning}
\usetikzlibrary{3d} %for including external image 

\def\DcnvColor{rgb:blue,5;green,2.5;white,5}

\begin{tikzpicture}
\tikzstyle{connection}=[ultra thick,every node/.style={sloped,allow upside down},draw=\edgecolor,opacity=0.7]

\pic[shift={(0,0,0)}] at (0,0,0) {RightBandedBox={name=cr1,fill=\DcnvColor,bandfill=\DcnvColor,%
        height=40,width={2,2},depth=40}};

\end{tikzpicture}
